TextGAIL: Generative Adversarial Imitation Learning for Text Generation

Generative Adversarial Networks (GANs) for text generation have recently received many criticisms, as they perform worse than their MLE counterparts. We suspect previous text GANs' inferior performance is due to the lack of a reliable guiding signal in their discriminators. To address this problem, we propose a generative adversarial imitation learning framework for text generation that uses large pre-trained language models to provide more reliable reward guidance. Our approach uses contrastive discriminator, and proximal policy optimization (PPO) to stabilize and improve text generation performance. For evaluation, we conduct experiments on a diverse set of unconditional and conditional text generation tasks. Experimental results show that TextGAIL achieves better performance in terms of both quality and diversity than the MLE baseline. We also validate our intuition that TextGAIL's discriminator demonstrates the capability of providing reasonable rewards with an additional task.

==> tables.tex <==
\section{Experiments}



\begin{table}[h]
    \centering
    \resizebox{0.8\textwidth}{!}{
    \begin{tabular}{ccccccc}
        \toprule
         Models & SeqGAN & LeakGAN & SAL & RelGAN & GPT2+MLE & TextGAIL\\
         \midrule
         Perplexity $\downarrow$ & $307.2$ & $291.4$ & $231.3$ & - (*) &  \textbf{20.82} & \textbf{20.82} \\
         \midrule
         BLEU-4 $\uparrow$ &  $0.307$ & $0.353$ & $0.362$  & $0.502$  & \textbf{0.860} & \textbf{0.860} \\
         \bottomrule
    \end{tabular}
    }
    \newline
    \caption{Results of COCO Image Captions.
    *We couldn't reproduce the model, and the original paper did not report perplexity.
    }
\end{table}

% \begin{table}[h]
%     \centering
%     \resizebox{0.8\textwidth}{!}{
%     \begin{tabular}{ccccccc}
%         \toprule
%          Models & SeqGAN & LeakGAN & SAL & RelGAN & GPT2+MLE & TextGAIL\\
%          \midrule
%          Perplexity $\downarrow$ & $743.8$ & $491.7$ & $612.8$ & - (*) &  \textbf{19.50} & \textbf{19.50} \\
%          \midrule
%          BLEU-4 $\uparrow$ &  $0.261$ & $0.437$ & $0.281$  & $0.501$  & \textbf{0.592} & \textbf{0.860} \\
%          \bottomrule
%     \end{tabular}
%     }
%     \newline
%     \caption{Results of EMNLP2017 WMT news generation.
%     *We couldn't reproduce the model, and the original paper did not report perplexity.
%     }
% \end{table}

\begin{table}[h]
    \centering
    \resizebox{1.0\textwidth}{!}{
    \begin{tabular}{l|ccccc}
        \toprule
        & COCO & EMNLP2017 WMT &  SNLI & CommonGEN & ROCStories \\
        \midrule
        Condition generation & $\times$ & $\times$ & $\checkmark$ & $\checkmark$ & $\checkmark$ \\
        \midrule
        Vocabulary size & 4681 & 12,972 & 15,592 & 12,941 & 20,937 \\
        \midrule
        Average length & 11.36 & 27.03 & 7.45 & 10.97 & 10.59 \\
        \midrule
        \# of Training Samples & 10000 & 278,586 & 183,384 & 39,069 & 98,161 \\
        \bottomrule
    \end{tabular}
    }
    \newline
    \caption{Dataset Statistics.
    }
\end{table}
